Turbo: Opportunistic Enhancement for Edge Video Analytics

Edge computing is being widely used for video analytics. To alleviate the inherent tension between accuracy and cost, various video analytics pipelines have been proposed to optimize the usage of GPU on edge nodes. Nonetheless, we find that GPU compute resources provisioned for edge nodes are commonly under-utilized due to video content variations, subsampling and filtering at different places of a pipeline. As opposed to model and pipeline optimization, in this work, we study the problem of opportunistic data enhancement using the non-deterministic and fragmented idle GPU resources. In specific, we propose a task-specific discrimination and enhancement module and a model-aware adversarial training mechanism, providing a way to identify and transform low-quality images that are specific to a video pipeline in an accurate and efficient manner. A multi-exit model structure and a resource-aware scheduler is further developed to make online enhancement decisions and fine-grained inference execution under latency and GPU resource constraints. Experiments across multiple video analytics pipelines and datasets reveal that by judiciously allocating a small amount of idle resources on frames that tend to yield greater marginal benefits from enhancement, our system boosts DNN object detection accuracy by $7.3-11.3\%$ without incurring any latency costs.

==> tex/design.tex <==
\section{Design Overview}
\label{sec:overview}
% OPIE targets to select the best IE-model for input images to improve overall accuracy within latency constraints. To achieve this, it need to solve three challenges: (1) which samples need to be enhanced? (2) which IE models should be used for a selected sample? (3) which execution policies should be used to meet latency bounds.

% To address first two challenges, we leverage multi-exit GAN architecture to build the detection-aware IE model for downstream object detection tasks. Benefiting from adversarial training, we not only get an GAN based IE model but also get an accurate image-level discriminator, which can predict the difficult score for an input image. In addition, our GAN-based IE model is not for general image enhancement tasks and is responsible for transforming hard images of the downstream detector to easy images for post-processing. Because we limit the enhancement’s difficulty from general to detector-specific, it is easy to learn semantic correspondence matching between easy and hard samples. With trained detection-aware IE model and a image-level discriminator, we profile accuracy gain and latency using different enhancement layers and execution policies on historical data, which can be used for latter online scheduling.

% When a new buffer of frames are fed into OPIE, we will execute the image-level discriminator to assign a difficult score to each one. Then an novel accuracy-optimized scheduling algorithm is proposed to find the best enhancement strategy for each image and the best execution policy for this buffer, which aims to achieve the maximum accuracy gain satisfying latency bounds.

% As illustrated in the Figure 1 \yan{(overview)}, OPIE consists of offline ($\S$\ref{subsec:ie}) and online ($\S$\ref{subsec:scheduler}) stages. Next, we will describe the key techniques of every stage in detail.

\begin{figure*}[!htb]
	\centering
	\includegraphics[width=2.0\columnwidth]{Images/OPIE_overview.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
% 	\vspace{-10pt}
	\caption{\name system overview. \yan{Update enhancement profiling with continuous functions}, \sq{1)Connect $G$ into online phase, 2) update $D$ in the online phase}}
% 	\vspace{-10pt}
	\label{fig:overview}
\end{figure*}

% --------------------------\\


Design of \name consists of a novel GAN-based image enhancement module and an online execution scheduler which runs the module on selected frames under a given resource budget so as to maximize the overall detection accuracy, as shown in Figure~\ref{fig:overview}. \sq{online phase and offline phase, the major modules or phases should be corresponded with Fig.5.}

\name's image enhancement module builds on top of recent advances in generative adversarial networks (GAN). Unlike traditional general GAN-based image enhancement, \name proposes a task-driven multi-exit GAN architecture and a model-aware adversarial training mechanism (\S\ref{subsec:ie-training}) \sq{more details and explanations on task-driven GAN}, which efficiently build a multi-exit GAN tailored for object detector used in a video analytics pipeline \sq{how about putting multi-exit into the latter paragraphs.}. Such a design not only makes it easy to learn semantic correspondence matching between easy and hard samples \sq{easy and hard, high-quality and low-quality, please unify the term}, yielding a reliable image classifier to determine frames that are more amenable to enhancement, but also reduces GAN model training complexity and inference latency. \sq{more explanations why task-driven model can reduce training complexity?} %In short, the holistic design allows our image enhancement to scale both horizontally - complementing with different object detection models without knowing much about their architectures and weights - as well as vertically by effectively learning from various enhancement models.

\sq{I suggest we can talk about task-driven or detector-specific image enhancement first, then discuss the multi-exit design in the latter paragraph, followed by the scheduler design.}

\name's scheduler takes as input the pre-trained GAN enhancement model as well as offline accuracy and cost profiling results (\S\ref{subsec:ie-profiling}) \sq{In Fig.5, there is no image enhancement module in online phase}, and decides on-the-fly how the multi-exit GAN is executed on frames so as to maximize the overall object detection accuracy. Due to video content variations and subsampling of video analytics pipeline, heavyweight object detection workloads vary over time and will likely under-utilize the GPU resources provisioned upfront for most of the time. Thus, within a given time frame, \name's scheduler firstly determines the resource budget by quantifying the number of frames reaching the object detector, and then uses the GAN discriminator to classify frames provided by upstream pipeline. Based on the classified difficulties and resource budget, a combinatorial optimization problem is formulated to decide how the enhancement model is executed at various levels on different frames. 

% In \name, we train a generalized GAN on BDD100K~\cite{yu2020bdd100k} and fine-tune its discriminator on testing data. In fine-tuning stage, we run an pre-trained object detection model on testing data and select hard samples based on its predicted confidences. Because the discriminator only needs to know which samples are hard, we train it without any annotations. More details can refer to \S\ref{subsec:ie-training}.
\sq{I suggest here we can brief the GAN is trained (on which dataset) and add the discriminator fine-tuning details. In Fig.5 add the discriminator fine-tuning part.}

\section{GAN-based Image Enhancement}
\label{sec:ie}
% \subsection{GAN-based Image Enhancement}
% \label{subsec:ie-gan}
% \yan{(GAN intro → why we choose GAN and adversarial training?)}

GAN~\cite{goodfellow2014generative, zhu2017unpaired, karras2019style,isola2017image} is a widely used neural network for image enhancement and synthesis. Unlike rule-based methods~\cite{Zamir2021MPRNet,zeroDCE2020guo,qin2020ffa,liang2021swinir}\sq{It might be not accurate to name the previous work 'rule-based'}, GAN adopts adversarial training~\cite{goodfellow2014generative} to learn a \emph{generator} ($G$) and a \emph{discriminator} ($D$) simultaneously. 

In GAN-based image enhancement, $G$ is responsible for generating synthetic high-quality images, whereas $D$ takes as input both synthetic and real high-quality images, and is trained to distinguish between these two sources.
Since $G$ and $D$ play a competing and continuous game, in which $G$ is learning to produce more and more realistic high-quality images, and $D$ is learning to be better and better at distinguishing synthetic data from real data, GAN-based image enhancement gains both generative and discriminative abilities at the end of training~\cite{jiang2021enlightengan,liang2021swinir,ganIE2021pan,ganIE2019li,ganIE2020du}. 
% In other words, it can not only transform low-quality images to high-quality ones, but also classify between these two categories. Naturally, 
Such ability well serves the purposes of identifying and transforming hard frame samples to ones that are more amenable to the object detector in the video analytics pipeline.
% Because IE-based video analytics systems require to decide which images should be enhanced and D is able to discriminate which images are hard ones, we choose GAN as our IE model. 

% \yan{(Limitations of GAN-based IE → why we need a detection-driven multi-exit GAN architecture and a model-aware adversarial training mechanism?)}
Despite superior accuracy, GAN training and inference are known to be challenging~\cite{weng2019gan}. The reason is two-fold. First, the definition of image quality vary significantly in different video ML tasks, and the need of having a \emph{general}, \emph{large-capacity} GAN-based enhancement model imposes great difficulties on design of both model architecture and adversarial leaning~\cite{Zamir2021MPRNet,zeroDCE2020guo,qin2020ffa,liang2021swinir,jiang2021enlightengan}. In fact, vanilla GAN enhancement models trained on public datasets~\cite{jiang2021enlightengan,liang2021swinir,ganIE2021pan,ganIE2019li,ganIE2020du} typically end up being an overkill to the downstream object detection task. For instance, a model trained from low-illumination images could bring negative impacts to Swin-Transformer-based detector~\cite{swin2021liu}), which performs exceedingly well in low-light scenarios~\cite{deep2018cai,fivek2011vladimir}.\sq{Very unclear what is the first issue, requiring the large dataset? need costly training? having negative impacts on detections?} Second, prohibitively high training and inference cost also hinders real-world deployment of GAN. Growing size of the model incurs higher labeling cost, and makes it harder for $G$ to converge during training. In addition, the stacked up-sampling layers in the encoder-decoder architecture also adversely impact inference latency. \sq{Not make sense to me for this issue. why high cost for training is a issue? Existing methods make it converge during training. What is stacked up-sampling layers? what are encoders and decoders? Brief the terms when they appear in our paper first time.}

\sq{Before present our solution, we can first discuss why we can do in this way...}
In \name, we propose a \emph{detector-specific} GAN architecture and a \emph{model-aware} adversarial training mechanism to cope with the above issues. As opposed to building a \emph{general purpose} model, our GAN architecture is tailored for the specific object detection model used in a video analytics pipeline. As such, we effectively reduce the complexity of GAN training by focusing only on images that are of low quality to one object detection model. To further reduces training and inference cost, we replace the encoder in $G$ with backbone layers of the detector since the latter has already been trained for extracting feature embedding \sq{we have two designs to reduce the training cost and inference cost, respectively. Destribe them one by one. To reduce the training cost, we reuse the backbone network for the encoder of $G$. To reduce the inference cost, we provide the multi-exit design?}.In addition, we adopt a multi-exit architecture~\cite{lin2021anycost} to provide more flexibility and fine-grained trade-off between inference latency and accuracy. \sq{More explanations on how we do this?}


% \ys{We need to fit Figure~\ref{fig:processing} into the context.}\yan{The second paragraph above introduced details about data pre-processing and I think this figure cannot provide much more information. Thus, can we remove this directly?}
% Although GAN provides G and D simultaneously, using vanilla GAN-based IE~\cite{jiang2021enlightengan,liang2021swinir,ganIE2021pan,ganIE2019li,ganIE2020du} in video analytics is not suitable for the downstream object detection task because the “easy-to-hard” semantic relationship is very different in IE and object detection models. In IE, models target to learn a general “easy-to-hard” transformation which should be effective to any corrupt image caused by an image noise~\cite{Zamir2021MPRNet,zeroDCE2020guo,qin2020ffa,liang2021swinir,jiang2021enlightengan}. For example, a GAN-based IE for low-light images will improve the visibility of any low-light images. But for object detection models, hard images are randomly distributed in low-light images and some recent models even (\eg Swin-Transformer~\cite{swin2021liu}) achieve remarkable performance on low-light images~\cite{deep2018cai,fivek2011vladimir}. Thus, the “easy-to-hard” semantic relationship should be detector-specific~\cite{xin2021detection} \yan{(from my opinion, model-aware may be misleading because we hope to highlight IE is specific to the downstream detection model)} to the downstream object detection task. To achieve this target, we create a detector-specific training data as illustrated in Figure~\ref{fig:processing} and use it to make GAN generate synthetic easy samples for the pre-trained object detection model. With a trained IE, we only get synthetic easy images, but it is still uncertain that they are effective for improving accuracy of the detector. To control the synthesis performance, we add a detection loss in the vanilla adversarial training process, which drives G to generate “easy-to-detect” images. 
% Besides, the training and the inference cost of GAN also prohibit real-world deployment because G is hard to convergence and its many stacked up-sampling layers are such time-consuming. By analysing main components of G, we find that G of GAN is based on an encoder-decoder architecture, where the encoder firstly extracts the feature embedding from an input image and the decoder uses up-sampling layers to restore semantic details from this embedding. Thus, a better encoder (or a good feature embedding) can speed up learning speed of G. Fortunately, backbone layers of pre-trained detectors are also responsible for extract effective feature embedding for post-processing. Thus, we use backbone layers to replace the encoder module of G to achieve fast convergence. To speed up inference speed, we integrate our GAN with a widely used multi-exit mechanism~\cite{lin2021anycost} in an effective way.

% As described in xxx, we cannot decide which images are hard and which image distortions a hard image belongs to. Thus, learning a classifier and a general IE model is required. Fortunately, we find that GAN is a such suitable model for this need due to its implicit modeling and adversarial-based training. GAN~\cite{goodfellow2014generative, zhu2017unpaired, karras2019style, isola2017image} is a widely used neural network in image synthesis and editing. It aims to train a generative network (G) to synthesis a new image from a random noise or an input image with help from a discriminative network (D). In training, it adopts the two-player non-cooperative game and trains the two components in a adversarial learning way. The standard GAN loss function is the min-max loss ($V$)~\cite{goodfellow2014generative}:
% \begin{equation}
%     \begin{split}
%     \mathop{min}_{G}\mathop{max}_{D}V(D, G) &= \mathbb{E}_{x\sim p_{data}(x)}[log D(x)]\\ 
%     & + \mathbb{E}_{z\sim p_{z}(z)}[log(1-D(G(z))]
%     \end{split}
%     \label{eq:ganLoss}
% \end{equation}
% where $p_{data}(x)$ and $p_{z}(z)$ represent distributions of training data and input noise respectively. In image editing applications (\eg{ IE}), we replace input noise with raw images. 

% When the training phrase is completed, we can get G and D simultaneously. Because D is able to classify which images are from real data and synthetic data, it can be used as a easy-hard classifier for IE models. Unlike collecting easy-hard samples caused by a single image distortion, GAN [] accepts easy-hard samples from mixed image distortions. Thus, it is more suitable for IE-based video analytics.

% However, training GAN is not easy and cost of inference with GAN is 2-3 orders of magnitude than existing CNN based IE models. Adversarial training always requires that G is collaborating with D in many cycles. At the beginning of the training phrase, G is too weak to generate reasonable outputs for D. Thus, a better D will provide G better matching signals. Unfortunately, if we set general easy-hard samples to training data, D is also hard to learn a good initialization at the beginning due to diverse easy-hard matching relations. To reduce the difficulty of D, we choose to learn detector-aware easy-hard matching relationship instead. Because easy-hard relationships can be modeling by hierarchical object detection models, we leverage multi-exit mechanism to speed up inference of GAN-based IE.

\subsection{Model-aware Adversarial Training}
\label{subsec:ie-training}
\sq{I suggest we should first highlight the key point of what is the detector-specific GAN?}
\sq{Also suggest we should firstly define what is the easy samples and hard samples. How we can differentiate them.,}
We first introduce our detector-specific GAN architecture, whose $G$ consists of an frozen encoder module (lock) and an trainable encoder (unlock) as shown in Figure~\ref{fig:overview_gan}. Because we expect it is tailored for the downstream object detection model, it should be capable of leveraging prior information from detectors and speeding up the end-to-end video analytics pipeline. To this end, we reuse a backbone module of the object detection model in $G$ to provide the \textit{detector-specific} feature embedding. Then an trainable up-sampling layers of $G$ will restore semantic details based on it.  \sq{Why we reuse the backbone, for speedup training or for detector-specific GAN?}
% in sequential processing. 
% Specifically, we denote an frozen backbone and trainable up-sampling layer of G by lock and unlock icons respectively in Figure~\ref{fig:overview_gan}.

\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.95\columnwidth]{Images/multiGAN_stage2.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
% 	\vspace{-10pt}
	\caption{An overview of our multi-exit GAN. In stage-1, we aim to pre-train GAN with $img^{hard}$ and $img^{easy}$, where $img^{hard}$ denotes synthetic images generated by the generator and $img^{easy}$ represents real easy images from training data. In stage-2, we target to learn the multi-exit mechanism of GAN with detection loss. In all stages, we reuse backbone layers of the downstream object detection model as an encoder module for the generator, and only update layers of a decoder module of the generator and two-level discriminators (unlock icon). \sq{the elements in this figure look very similar and repetitive with Fig.5. Try to revise this figure or simplify Fig.5?}}
% 	\vspace{-10pt}
	\label{fig:overview_gan}
\end{figure}

The overall architecture of $G$ is based on U-Net~\cite{2015unet} which fuses low-level feature maps into high-level up-sampling layers to generate more realistic images. But naively using $G$ as data pre-processing for the specific object detection model in a video analytics pipeline is much costly because we have to run a full $G$ on every image \sq{To claim if $G$ is costly, give an example and show real number.} \sq{I think the key point here is not whether it is costly or not, but we should enable an elastic structure to fit the resource dynamics}. To build a more efficient execution pipeline, we add a \textit{detector-specific} multi-exit mechanism to up-sampling layers of G. \sq{we have discussed detector-specific, here we can just talk about multi-exit.} In specific, enhanced feature maps of the $k_{th}$ layer of the up-sampling module will be sent to the $k_{th}$ layer of the downstream backbone module.\sq{More details and explanations.}
% Unlike other exiting mechanisms on GAN, we don't use it to generate synthetic images with different resolutions and we use it to generate enhanced feature maps for the downstream object detection model.
% the output enhanced feature maps instead of raw images to the downstream backbone module. 
% can be seen as feature enhancement on the $k_{th}$ layer of backbone. 
% In specific, we will send enhanced feature maps from the $k_{th}$ layer of up-sampling module to the $k_{th}$ layer of downstream backbone module. 
In $D$, we follow a popular two-level discriminator~\cite{jiang2021enlightengan,ganIE2021pan} to design image-level and instance-level classifiers for discriminate synthetic images and bounding boxes respectively. \sq{unclear, more details must be added. why we need this? how this two-level design help solve our problem?}
% Then
% two feature maps from the $k_{th}$ layer of backbone and the $(k-1)_{th}$ layer of up-sampling module are inputted and then enhanced feature maps for the $k_{th}$ layer of backbone are generated. Thus, each up-sampling layer is responsible for transforming raw feature maps of its corresponding backbone layer to enhanced ones based on high-level semantic features provided by the previous up-sampling layer. In D, we follow a popular two-level discriminator~\cite{jiang2021enlightengan,ganIE2021pan} to design image-level and instance-level classifiers for discriminate synthetic images and bounding boxes respectively.

To train our GAN, a two-stage \textit{model-aware} adversarial training mechanism is proposed: (1) model-aware adversarial training and (2) supervised training on multi-exit feature enhancement. Because early exits from G are responsible for improving feature maps instead of the raw image, we train G without multi-exit mechanism and D in Stage 1. With supervised signals from labeled images, we fine-tune G with all exits and D in Stage 2. As shown in Figure~\ref{fig:overview_gan},
we also add a adversarial loss as an regularization term to preserve G's ability on image-level enhancement in Stage 2 . 
% Without a good initialization on G in Stage 1, Stage 2 will need more time to convergence and will be hard to find the optimal weights for G. It's because that optimization in a single adversarial training is often unstable and limited by local minimal. Also, adding $L_{det}$ to a weak G directly cannot help minimize $L_adv$. But in contrary, a good G will help us minimize $L_{det}$ because G has learned coarse-level detector-specific information from minimizing $L_adv$. 

% An alternative method is training G with $L_adv$ only and then fine-tune it with the overall loss $L$.

\sq{I suggest we could move some of following contents ahead. Overall to train a GAN, we need the paired samples, how do we define them, where are they from.}
To achieve model-aware adversarial training, we do not assume that there exists a dataset with labeled easy and hard images for adversarial training. Instead, we collect \textit{detector-specific} easy and hard samples based on image-level confidence scores predicted by the pre-trained object detection model. In specific, we compute the image-level score by averaging confidence scores of all RoIs in an image, and select images with low image-level confidence score as hard images and the remaining as easy samples. \yan{It is because we find that many region-of-interests (RoIs) in hard frames are localized by object detectors correctly but are assigned to low confidence.} In adversarial training, G will transform raw hard images to synthetic easy ones. Then image-level D will distinguish the real easy images from the fake generated easy images. Besides, we run the specific detector on two easy images and use its outputs (bounding boxes) as inputs for instance-level D. In sum, the adversarial loss $L_{adv}$ function can be formulated as: \sq{How about giving the meaning of this loss function first?}
\begin{equation}
    \begin{split}
        L_{adv} &= \mathbb{E}_{x\sim p_{data}(x)}[log D_{img}(x)] + \mathbb{E}_{x\sim p_{data}(x)}[log D_{ins}(x)]\\ 
        & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{img}(G(z))] \\
        & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{ins}(G(z))]
    \end{split}
    \label{eq:IELoss}
\end{equation}
where $p_{data}$ denotes the data distribution mixed by real and synthetic easy images, and $p_{hard}$ represents the distribution of hard images. \yan{To achieve more generalized model-aware adversarial training, we need a more robust hard samples selection strategy. For example, it is easy to split }
% $L_{det}$ is an standard loss function of object detection. 

Without any information about how the specific detector perform on synthetic images, it is hard to learn feature-level enhancement. In other words, $L_{adv}$ only tells G the final generated images are not good but G cannot infer which up-sampling layers work bad\sq{what is up-sampling layers? Why do we need to know which layer works not well? If here we have already introduced the multi-exit arch, then we only describe how the multi-exit is trained, that's all}. Thus, supervised signals from labeled hard images are required in Stage 2. For a hard image, we expect all exits should be effective to improve its semantic details for a final higher detection results. Thus, we first compute loss for each exit by comparing its predictions and the label for an given hard image. Then, we get the final detection loss via averaging losses of all exits. Because a single supervised signal is not enough to preserve G's image-level enhancement ability, we add $L_{adv}$ to the training process as an regularization term. In sum, the overall loss $L$ function of Stage 2 is:$$L=\frac{1}{5}\sum^{5}_{k=0} L^{k}_{det}+L_{adv}$$\sq{1/5 is not reasonable.} where $k$ denotes the exit's index and $L_{det}$ is an standard loss function of object detection.

Because Stage 1 doesn't need any annotations and Stage 2 requires labels of hard images, our training can be seen as a semi-supervised training method. In experiments, we find that labeling of $25\%$ hard samples in Stage 2 is sufficient to generate decent enhancement performance.\sq{show real number or figures here. Instead of a plain number, we need to show some insights, e.g., the more hard samples, the better results? How about 100\% hard samples? Why 25\% is a golden number, why not 20\%? Instead of the ratio, what about the absolute amount of data?}

\sq{We can talk about the dataset used to train the GAN, what is our data selection policy for the training? Why can we do in this way?}
% \begin{equation}
%     \begin{split}
%         L_{adv} &= \mathbb{E}_{x\sim p_{data}(x)}[log D_{img}(x)] + \mathbb{E}_{x\sim p_{data}(x)}[log D_{ins}(x)]\\ 
%         & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{img}(G(z))] \\
%         & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{ins}(G(z))]
%     \end{split}
% \end{equation}

% \ysedit{
% To learn a semantic "easy-to-detect" G, we devise a two-stage adversarial training method: (1) GAN pre-training with pseudo labels, and (2) multi-level feature enhancement learning. Stage 1 aims to train a generator to synthesis semantic easy images, and stage 2 targets to make G generate easy-to-detect images for the detector down the pipeline (Figure~\ref{fig:overview_gan}). \ys{Unclear what are the differences between two stages.}

% Unlike previous GAN-based image enhancement methods~\cite{jiang2021enlightengan,liang2021swinir,ganIE2021pan,ganIE2019li,ganIE2020du}, we do not assume that there exists a dataset with labeled easy and hard images for adversarial training. Instead, we collect detector-specific easy and hard samples based on image-level confidence scores predicted by the pre-trained object detection model. In specific, we compute the image-level score by averaging confidence scores of all RoIs in an image, and select images with low image-level confidence score as hard images and the remaining as easy samples.
% %Intuitively, images with low confidence should be harder for the detector. 
% In experiments, we follow the settings in existing works~\cite{guo2020multiscale,jin2018semiod,xin2021detection} and set the threshold to $0.5$. 

% As described above, synthesising "easy-to-detect" images requires supervised signals from a detection loss. Thus, \ys{in stage 2?}, we collect annotations by hand-labeling hard images and pseudo-labeling easy images using the detector. We find in our experiments that labeling of $25\%$ \ys{of what?} is sufficient to generate decent enhancement performance. %Note that we only need to label hard frames manually because incorrect pseudo-labels on easy images are not effect GAN's training (we hope GAN can be capable of transforming hard images to easy ones. Thus, ground-truths for hard are required because we need to know the optimization's trend of GANs is matching our expectations. But for easy images, we choose to skip all enhancement layers and thus don't need their annotations as supervised signals).

% % with help from the downstream object detection model. In adversarial training, there are two stages: (1) model-aware adversarial training and (2) multi-level feature enhancement learning. The first one aims to train a detector-aware generator for the downstream object detection model and the second one targets to modeling easy-hard relationship between the GAN and detector. The overview of model-aware adversarial training is illustrated in Figure~\ref{fig:overview_gan}.

% % Prior to adversarial training, we collect hard and easy images from the pretrained object detection model at first. After running the detector on each image, we get a confidence-score for each Region-of-Interest (RoI) and compute the average confidence-score for each image as its hard-score. Refer to many object detection models [], we use 0.5 as threshold to group easy and hard data. The details can be found in Figure~\ref{fig:processing}. Because multi-level feature enhancement learning requires labeled data and easy samples are not required to be enhanced by IE, we collect annotations of hard samples manually and use pseudo-labels from the detector on easy samples directly. 

% % \begin{figure}[!t]
% % 	\centering
% % 	\includegraphics[width=1.0\columnwidth]{Images/data_preprocessing.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
% % % 	\vspace{-10pt}
% % 	\caption{Data preprocessing for model-aware adversarial training.}
% % % 	\vspace{-10pt}
% % 	\label{fig:processing}
% % \end{figure}

% % \begin{figure*}%
% %     \centering
% %     \subfloat[\centering Stage-1: GAN training with two-level discriminator]{{\includegraphics[width=0.9\columnwidth]{Images/multiGAN_stage1.pdf}\label{fig:stage-1}}}%
% %     \qquad
% %     \subfloat[\centering Stage-2: End2end training with detection loss]{{\includegraphics[width=0.9\columnwidth]{Images/multiGAN_stage2.pdf}\label{fig:stage-2}}}%
% %     \caption{An overview of our multi-exit GAN. In stage-1, $img^{hard}$ denotes synthetic images generated by the generator and $img^{easy}$ represents real easy images from training data. In stage-2, we omit details in the discriminator. In all stages, we reuse backbone layers of the downstream object detection model as an encoder module for the generator, and only update layers of a decoder module of the generator and two-level discriminators (unlock icon).}%
% %     \label{fig:overview_gan}%
% % \end{figure*}



% Vanilla GANs are likely to suffer non-convergence issue due to the imbalance of \ys{what}~\cite{gan2019hoang,gan2018fedus} \yan{capacity} between G and D. In most cases, it is easy to learn a decent binary classifier D. \yan{However, a so strong D leads a vanishing gradient problem~\cite{weng2019gan}, where G is hard to use D's feedback to make improvements because D will tell each time there is a fake image. Without any supervised signals on cheating D, G is easy to confuse what its optimization target is.}\ys{confusing sentence}. An alternative method to improve G is to assign a good initialization like many transfer learning works~\cite{gan2020hu,transfer2019maithra}. Unfortunately, a GAN-based image enhancement trained on public image enhancement datasets~\cite{deep2018cai,fivek2011vladimir,iedata2017eirikur} is not suitable for our needs. Concretely, an existing image enhancement dataset is often targeting to one or two specific tasks of image restoration (\eg de-blurring and de-noising). But for dynamic video contents, we need to handle multiple noise simultaneously. Thus, a GAN-based image enhancement model pre-trained on public datasets are not suitable for our tasks.\yan{"general" is misleading and I use "public" to replace it.} \ys{what is the logic between a good initialization and a general dataset?} Thus, finding a good initialization for G is a key to adversarial training in stage-(1). To alleviate learning burdens of G, we replace an encoder module of G with backbone layers from the detector. Because backbone layers are able to extract effective feature embedding, we freeze them (lock) and only update the decoder module (unlock) in the training phrase as shown in Figure~\ref{fig:overview_gan}. \yan{With a enough good embedding, G can synthesis some synthetic images matching to real distributions of easy images. Thus, these generated images will fake D and adversarial training will return positive feedbacks to G. After comparing positive and negative feedbacks, G will be more clearly which targeting distribution is meeting D's requirement.} \ys{similarly, how reusing backbone layers helps initialization?} Additionally, we use two discriminators instead of a single image-level discriminator because the new instance-level classification prevents the whole discriminator from overfitting to image-level features~\cite{jiang2021enlightengan}, which as a result leads to a better balance of \yan{capacity}\ys{what} between G and D.

% % In stage-1, we use backbone layers our generator $G_{IE}$ 
% % based on backbone layers of the downstream object detection model. G from vanilla GANs are based on encoder-decoder architecture, which extracts hierarchical features from inputs and then uses up-sampling modules to recover output from extracted feature embeddings. Given a object detection model, its backbone layers are also responsible for extracting features for post processing. Thus, we reuse backbone layers of the detector as G’s encoder module, which not only provides a good feature embeddings for G but also helps us to build multi-level feature enhancement in stage-2. In training, G is responsible for transforming hard images to synthetic easy images and our discriminator $D_{IE}$ needs to discriminate which images belong to real easy images from synthetic ones. As shown in Figure~\ref{fig:stage-1}, we use image-level and instance-level discriminators concurrently to avoid model collapse caused by xxx. 
% % \yan{in progress}

% Generator G obtained at the end of stage-(1) is only capable of generating semantic easy images for the detector. Hence, to make sure the enhanced images boost detectors' performance, we add the detector as GAN's downstream task and use supervised signals from labeled data to lead G synthesis "easy-to-detect" images. Specifically, we link the last layer of G to the first layer of the detector and compute the loss between predicted and labeled RoIs. Because we only want to learn GAN-based IE, we freeze all layers of the detector as illustrated in Figure~\ref{fig:overview_gan}.
% }

% To speed up inference, we add a multi-exit mechanism between G and backbone layers of the detector. Unlike existing works \yan{only add multi-exit to a single model}, we revisit inference's efficiency from a pipeline perspective and find that images are distorted in earlier layers should be hard images because it will make bad feature maps propagate in the whole DNN. Thus, if an image are difficult to be extracted correct semantic features at the $1^{st}$ layer should be harder than the $5^{nd}$ layer. Based on this finding, we link the $k^{th}$ layer of G’s decoder (yellow layers in Figure~\ref{fig:overview_gan}) to the $6-k^{th}$ layer of the detector. \ys{not clear what's new here.} \yan{Although there are many works about multi-exit GANs, they only use the exiting mechanism to speed up GAN instead of speeding up the whole pipeline (GAN + DNN). Thus, I think linking suitable exits to downstream detectors' layers is not trivial to the community.}

% % follow the multi-exit mechanism and add a exit to each layer. Based on hierarchical design of object detection models, feature maps of hard images should be distorted in earlier layers and make bad end-to-end performance. For example, if an image are difficult to be extracted correct semantic features at the $1^{st}$ layer should be harder than the $5^{nd}$ layer. Thus, we link the $k^{th}$ layer of G’s decoder (yellow layers in Figure~\ref{fig:overview_gan}) to the $6-k^{th}$ layer of the detector.

% \textbf{Put it all together}. The overall loss function of two stages $L$ can be formulated as:
% \begin{equation}
%     \begin{split}
%         L &= \mathbb{E}_{x\sim p_{data}(x)}[log D_{img}(x)] + \mathbb{E}_{x\sim p_{data}(x)}[log D_{ins}(x)]\\ 
%         & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{img}(G(z))] \\
%         & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{ins}(G(z))] + L_{det}
%     \end{split}
%     \label{eq:IELoss}
% \end{equation}
% where $p_{data}$ denotes the data distribution mixed by real and synthetic easy images, $p_{hard}$ represents the distribution of hard images and $L_{det}$ is an standard loss function of object detection. 
% \ys{feels it's incomplete. we should either expand this part with more details or totally remove it.}

\subsection{Enhancement Profiling}
\label{subsec:ie-profiling}
\sq{I suggest we could move this subsection into the scheduling part, since the profiling results are used for scheduling.}

\sq{more details are needed}
In order to determine the best exit layer during enhancement execution under resource constraints, we need to get a sense of the accuracy-resource tradeoff of running the pre-trained GAN model at different levels on GPU. To do so, we introduce an offline profiling step. In specific, we bucketize images based on their difficulty scores obtained from the previous step, and record average accuracy by running the enhancement model at different levels on each set of images. This way, we are able to estimate the enhancement performance of a particular image by mapping its difficulty to a pre-calculated difficulty-accuracy profile. In terms of resource consumption, we run different levels of the enhancement model with respect to various batch sizes in an exhaustive manner, and record corresponding inference latency numbers. Note that this is a one-time effort and the latency results hold true for online scheduling as they are independent of frame content. 

% \yan{Although a pre-trained G and D are effective to help us select enhancement plan in runtime, both of them are working on frame-level. In online, selecting suitable enhancement layers is not only correlate with video contents but also dynamic idle resources. Thus, a better solution should not only select a good enhancement layer for an image but also select all enhancement layers for a group of images. To achieve this, we profile accuracy-latency of G and using them to select suitable enhancement plans from statistical perspective.}
% \ys{We need to talk about why profiling is needed first and then how we do it.}
% With trained $G$ and $D$, we first profile accuracy of using different feature enhancement layers to enhance images belonging to the same range of predicted difficult-score. The profiling process is a one-time effort and we can run it in the offline phase. Specifically, the predicted image difficulty $D$ and selected the image enhancement based detectors $M$ are inputted to our accuracy profiling function $p(\cdot)$ and it outputs the overall accuracy $Acc$.  

% In online stage, $f(\cdot)$ takes a assignment plan $A$ as inputs, and compute the end-to-end execution's latency $L$ via summing all estimated latency of each $M$.
% Because profiling networks' inference latency needs to consider current idle resources, we execute many models concurrently and profile the end-to-end latency. Assuming the detector which exits at the $k_{th}$ enhancement layers of $G_{IE}$ is $m^{k}$. When $k^{max}=3$, we need to run 4 execution plans ($m^{1}\&m^{2}$, $m^{1}\&m^{3}$, $m^{2}\&m^{3}$ and $m^{1}\&m^{2}\&m^{3}$) under different batch sizes and then record their latency. Details can be found in Figure~\ref{fig:overview}. As same as $p(\cdot)$, the cost profiling function $f(\cdot)$ takes a assignment plan $A$ as inputs, and outputs the execution's latency $L$.

% \textbf{Put it all together.} In summary, two profiling functions are formulated as:
% \begin{equation}
%     \begin{split}
%         \bigtriangleup Acc &= p(M, D)\\
%         L &= f(M, E)\\
%     \end{split}
%     \label{eq:profiling}
% \end{equation}

% \section{Design}
% As described before, IE based video analytics require to select (1) which \textbf{samples} need to be enhanced? (2) which \textbf{IE models} should be used for a selected sample? (3) which \textbf{execution policies} should be used to achieve high resource utilization on idle resources. 

% Inspired by the implicit modeling characteristic of GAN and recent multi-exit GAN architectures~\cite{lin2021anycost} which can be executed at various computational cost budgets to meet different latency requirements, we build \textit{model-specific multi-exit GAN} to enhance intermediate features and outputs of an given object detection model. Benefiting from its two-player non-cooperative game in training, we can get not only an general IE model but also a sample discriminator which can select which new images are worthwhile to be enhanced. Moreover, the multi-exit design makes us run the IE model in a flexible way to meet dynamic idle resources. 

% To achieve high resource utilization on idle resources, we propose \textit{resource-aware scheduling} approach to select the optimal execution policy of IE models to achieve high resource utilization on idle resources. xxx
% % \yan{1. GPU measurement to find a suitable physical meaning for $y$ (resource budget); 2. Global control/scheduling to trade-off the sum of xxx usage $\sum^{i-1}_{i=0} y^{i}$ and the current difficult-level score $d^{i}$ with awareness of the variants of video contents (distributions of hard samples).}


% \subsection{Detection-specific Multi-Exit GAN}
% \subsubsection{GAN and its variants.}
% GAN~\cite{goodfellow2014generative, zhu2017unpaired, karras2019style, isola2017image} is a widely used neural network in image synthesis and editing. The aim is to train a generative network to synthesis a new image from a random noise or an given image. To achieve its target, researchers design two components (generator and discriminator) and train them in the two-player non-cooperative way, which is also named as adversarial training in machine learning community. In the training, a generator (\textit{G}) targets to generate new data from an given input to fit the distribution of training data (\eg{ high resolution images}) and a discriminator (\textit{D}) aims to discriminate between two (or more) different classes of data (\eg{ low and high resolution images}). Because G’s training objective is to increase the error rate of the discriminative network and D's aim is to reach some level of classification accuracy, the standard GAN loss function is the min-max loss ($V$)~\cite{goodfellow2014generative}:
% \begin{equation}
%     \begin{split}
%     \mathop{min}_{G}\mathop{max}_{D}V(D, G) &= \mathbb{E}_{x\sim p_{data}(x)}[log D(x)]\\ 
%     & + \mathbb{E}_{z\sim p_{z}(z)}[log(1-D(G(z))]
%     \end{split}
% \end{equation}
% where $p_{data}(x)$ and $p_{z}(z)$ represent distributions of training data and input noise respectively. In image editing applications (\eg{ image enhancement}), we replace input noise with raw images. 

% Unlike rule-based image enhancement techniques, GAN only needs to define general easy and hard samples in the training dataset instead of specific low-quality data (\eg{ low-light images}). Also, D from two-player training can be used as the sample selector to choose which images need to be enhanced. Thus, GAN is most suitable for IE based video analytics systems due to its advantages of automatic sample and IE model selection.

% However, GANs' cost is 2-3 orders of magnitude than other rule-based specific IE techniques. Thus, how to accelerate GAN based IE is a challenging issue to use GAN in IE based video analytics pipelines. Inspired by early exiting architectures~\cite{}, multi-exit mechanism is used for building a anycost GAN~\cite{lin2021anycost} which can outputs under various and fine-grained computation budgets. Unfortunately, existing GAN based IE techniques~\cite{} don't consider the performance of downstream vision tasks (\eg{ object detection}) and focus on optimizing enhancement performances only. But in IE based video analytics, we expect to use IE techniques to improve the overall accuracy of object detection. Thus, we design an detection-driven adversarial training framework to train GAN based IE model. In addition, we speed up the whole pipeline of IE based video analytics via backbone reusing, which not only makes inference more efficient but also speeds up convergence in the training stage.

% \yan{(1) Highlight GANs' characteristics (implicit modeling easy and hard samples, two-player non-cooperative game in training, multi-exit architectures support flexible execution pipelines) can be matched to requirements of IE based video analytics perfectly. (2) Unfortunately, existing GAN and its variants focus on optimizing image enhancement solely and they are not aiming to improve downstream tasks' performance. Although using the multi-exit mechanism make GAN output at flexible runtime budgets, they ignore global optimization techniques on IE based video analytics.} 
% \subsubsection{Detection-driven adversarial training.}
% Our IE model consists of two components ($G$ and $D$) as same as classic GANs. Usually, $G$ from existing works~\cite{} are based encoder-decoder architectures, which extracts hierarchical features from inputs and then uses up-sampling modules to recover outputs from extracted feature embeddings. Fortunately, backbone layers of object detection models are also responsible for extracting features for latter processing. Thus, we reuse backbone layers of the downstream object detection model as an encoder module of $G$, which not only provides effective feature embedding for $G$ but also helps us build more effective multi-exit feature-level enhancement for downstream object detection models. 

% Although multi-exit mechanism is effective to editing images at different computation budgets, all of them output the whole image at various resolution which leads to large computation burdens for video analytics pipelines because each image is always needed to processed by an IE model and object detection model jointly. To optimize inferences' efficiency from pipelines' perspective, we build the detection-specific multi-exit generative model, where the last exiting is responsible for synthesis enhanced images and other exiting gates are responsible for generate enhanced feature maps for a downstream detection model. As shown in Figure~\ref{fig:overview_gan}, images enhanced by only three layers (yellow) can skip the first two layers of a backbone module in the object detection model. 

% In $D$, we build image-level and instance-level dicriminators to help minimax training process more stable because a single image-level classifier is easily to overfit the binary classification dataset and it leads to a unequal game between two players. Moreover, the instance-level discriminator are more accurate than the image-level discriminator on assigning difficult-level to new images.  

% Before training, we split easy and hard images based on mean average precision computed on ground truths and predicted outputs from an given pre-trained object detection model. G's aim is to synthesis easy images from given hard images and D targets to discriminate between real and synthetic easy images. \footnote{In training, we assume that the annotations of all images are available.}  

% As presented in Figure~\ref{fig:overview_gan}, we freeze layers of object detection models (lock) and only update parameters of remaining layers of $G$ and two-level discriminators (unlock). To implement detection-specific enhancement, we add detection loss to the min-max loss function and the overall loss $L$ can be formulated as:
% \begin{equation}
%     \begin{split}
%         L &= \mathbb{E}_{x\sim p_{data}(x)}[log D_{img}(x)] + \mathbb{E}_{x\sim p_{data}(x)}[log D_{ins}(x)]\\ 
%         & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{img}(G(z))] \\
%         & + \mathbb{E}_{z\sim p_{hard}(z)}[log(1-D_{ins}(G(z))] + L_{det}
%     \end{split}
% \end{equation}
% where $p_{data}$ denotes the data distribution mixed by real and synthetic easy images, $p_{hard}$ represents the distribution of hard images and $L_{det}$ is an standard loss function of object detection. 

% \yan{Highlight co-training's contributions to building an efficient and effective IE based video analytics pipeline (backbone reusing, multi-exit feature enhancement and detection-specific enhancement).}
% \subsection{Resource-aware scheduling}
% xxx (ongoing)
% \yan{Because it is meaningless to discuss easy/hard samples (images) without downstream object detection tasks, we use the feature maps from the backbone module are whether good enough to decide images' difficult-level. Due to error propagation in layer-by-layer inference, bad feature maps will lead to poor performance in the final classification and localization tasks. Especially on a extremely hard image, the first feature map of backbone module may be too noisy to provide discriminative spatial contexts for post-processing. But for a simple image, adding a few spatial context to the feature map extracted by latter layers of backbone is a more reasonable method because of the limited number of noisy spatial contexts. Thus, we design a multi-exit GAN and train it in the detection-driven strategy. In the runtime, extremely hard images will be enhanced fully (the final layer of GAN) before downstream object detection tasks.}\\
% \name is a \textbf{plug-and-play} enhancement module for existing object detection models and contains two key components: (1) detection-driven image enhancement (offline), which can generate multi-scale enhanced images for feature maps extracted by backbone layers of off-the-shelf object detection models as shown in Figure~\ref{fig:overview_gan}; (2) dynamic enhancement selection (online), which is in charge of selecting different-capacity GAN modules for a new frame under given resource budgets as illustrated in Figure~\ref{fig:overview}. In our design, we assume that pre-trained backbone layers from detection models support the multiple existing strategy. In implementation, we add 5 existing gate to backbone layers. 

% \begin{figure*}[!t]
% 	\centering
% 	\begin{subfigure}
% 	\centering
%          \includegraphics[width=1.0\columnwidth]{Images/multiGAN_stage1.pdf}
%          \caption{$y=x$}
%          \label{fig: gan_stage1}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}
% 	\centering
%          \includegraphics[width=1.0\columnwidth]{Images/multiGAN_stage2.pdf}
%          \caption{$y=x$}
%          \label{fig: gan_stage2}
% 	\end{subfigure}
% 	\includegraphics[width=1.0\columnwidth]{Images/image_enhancement.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
% 	\vspace{-10pt}
% 	\caption{An overview of our multi-exit GAN.}
% 	\vspace{-10pt}
% 	\label{fig:overview_gan}
% \end{figure*}
% \begin{figure*}[!t]
% 	\centering
% 	\includegraphics[width=2.0\columnwidth]{Images/scheduling_design.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
% 	\vspace{-10pt}
% 	\caption{\name system overview.}
% 	\vspace{-10pt}
% 	\label{fig:overview1}
% \end{figure*}
% \subsection{Detection-Driven Image Enhancement}
% Given an pre-trained object detection model, we split it into backbone layers and detection heads\footnote{In two-stage object detection models, we named a group of region proposal networks (RPN) and detection layers as detection heads.}. Because we freeze the whole detection model during training, we add a "lock" icon to detection modules and a "unlock" icon to GAN modules in Figure~\ref{fig:overview_gan}. To present multi-exit GAN easily, we use $G$, $B$, $H$, $D_{img}$ and $D_{ins}$ to denote the \textbf{decoder} of generator, backbone, detection head, image-level and instance-level discriminator modules.
% \subsubsection{Multi-exit architecture}
% In our multi-exit GAN, we adopt U-Net~\cite{liu2018unet}, which preserves rich texture information and synthesizes high quality images using multi-scale context information, as our generator module. 
% As shown in Figure~\ref{fig:overview_gan} (denoted by purple rectangle), we use backbone layers as an encoder, and build five upsampling+CNN blocks as their decoder modules in the generator. Compared to other U-Net based enhancement models (\eg EnlightenGAN~\cite{jiang2021enlightengan}), we don't assume that models know main reasons (\eg low-light) of hard samples in advance. Thus, we don't leverage existing constraints (\eg illumination-based attention maps) to train our GAN.  
% \subsubsection{Unpaired detection-driven GAN training}
% \label{gan_training}
% To train our multi-exit GAN, we collect a large number of labeled images and divide them into easy and hard groups based on mean average precision (mAP) predicted by an off-the-shelf detection model. Given mAP on each image, we sort images in descending order and select top-75\% images as easy samples. The remaining 25\% images as hard samples. Like EnlightenGAN~\cite{jiang2021enlightengan}, our GAN's loss ($L_{GAN}$) contains two components (image- and instance-level) and can be formulated as:
% \begin{equation}
%     L_{GAN} = L^{img}_{GAN} + L^{ins}_{GAN}
% \end{equation}
% The loss function for the image-level adversarial learning is:
% \begin{equation}
%     \begin{split}
%         L^{img}_{GAN} & = E_{x\sim P_{data}(x)}[logD^{img}(x)] \\ 
%         & + E_{z\sim P_{hard}(z)}[log(1-D^{img}(G(z)))] 
%     \end{split}
% \end{equation}
% To achieve instance-level adversarial learning, we randomly extract 4 bounding boxes from easy samples and all bounding boxes from the output (enhanced images) each time as shown in Figure~\ref{fig:overview_gan}. Similar to $L_{img}$, the loss function of the instance-level adversarial learning is:
% \begin{equation}
%     \begin{split}
%         L^{ins}_{GAN} & = E_{x^{'}\sim P_{data}(x^{'})}[logD^{ins}(x^{'})] \\ 
%         & + E_{z^{'}\sim P_{hard}(z^{'})}[log(1-D^{ins}(G(z^{'})))]
%     \end{split}
% \end{equation}
% To reuse intermediate enhanced features for downstream detection tasks, we add average detection loss ($L_{DET}$) to constrain our generator ($G$) training:
% \begin{equation}
%     L_{DET} = E_{x\sim P_{data}(x)}[\frac{1}{5}\sum^{5}_{i=1}l_{det}(y, H(B^{6-i}(G^{i}(x))))]
% \end{equation}
% where $l^{det}$ denotes the classic detection loss and $y$ denotes ground-truths (RoIs' locations and categories). Because we leverage the correlation between backbone (encoder) and decoder layers to select skipping layers on post detection models, we add new skip connections between decoder and backbone layers as illustrated in Figure~\ref{fig:overview_gan}. For example, when we exit at the $i^{th}$ layer of decoder, we will input our enhanced feature maps (enhanced by $i$ layers of decoder) to the $(6-i)^{th}$ layer of backbone module. In summary, the loss of \name is written as:
% \begin{equation}
%     L_{\name} = L_{GAN} + L_{DET}
% \end{equation}
% In implementation, we first pre-train our GAN with only $L_{GAN}$ in few epochs and then train it with $L_{\name}$ in the end-to-end manner. 

% \ys{We don't need to talk about all the details of training, especially those well-known or standard steps. Instead, we need to focus on what's new in our design and how it helps reduce the training/inference cost or improve accuracy in our unique setup.}

% \ys{We need to talk about the training cost, and justify that it's, hopefully, not a high price we pay for image enhancement.}
% % \begin{equation}
% %     % \begin{aligned}
% %     \begin{split}
% %     L_{GAN} & = E_{x\sim P_{data}(x)}[logD^{img}(x)] + E_{x^{'}\sim P_{data}(x^{'})}[logD^{ins}(x^{'})]\\
% %     & + E_{z\sim P_{hard}(z)}[log(1-D^{img}(z))] \\
% %     & + E_{z^{'}\sim P_{hard}(z^{'})}[log(1-D^{ins}(z^{'}))]
% %     \end{split}
% %     % \end{aligned}
% % \end{equation}
% % \subsubsection{Inference (remove)}
% \subsection{Dynamic Enhancement Selection}
% % \vspace{-10pt}
% With an trained multi-exit GAN, we will execute enhancement layers adaptively under given resource budgets. To further cope with the dynamic resource budgets at runtime, \name has the following two objectives: 1) Given a new image, it need to predict the difficult-level accurately and find the most suitable exiting layer based on detection accuracy (mAP); (2) Given a resource budget (latency or flops), it dynamically adjust the former exiting strategy to achieve the best accuracy under new budgets. Before our design, we first introduce our simple but effective difficult-level prediction algorithm. As shown in Figure~\ref{fig:overview}, we add a $D_{ins}$ trained in Section~\ref{gan_training} to the outputs extracted from backbone layers. In two-stage object detection models (\eg Faster R-CNN), it is easy to leverage their RPN to search all RoI candidates and use $D_{ins}$ to predict difficult-level for each RoI candidate\footnote{For one-stage object detection models (\eg YOLOv3), we have to run all layers of object detection models to extract all RoI candidates.}. With predicted difficult-levels on all candidates of one image, we average all results and use it to represent difficult-level for this image. Because we only execute enhancement modules on hard samples, we set the threshold $T_{hard}$ and filter images whose difficult-levels less than $T_{hard}$.

% \subsubsection{Neural network (NN) profiling}
% With difficult-levels, it is straightforward to profile the characteristics of available networks, more specifically, their latency/flops-accuracy trade-off on different difficult-levels. The profiling process is a one-time effort and we can execute it in the offline phrase. After profiling, we will obtain performances of each exiting strategy on hard samples of different difficult-level intervals. For example, Table~\ref{table:profile_faster_rcnn} shows an NN profile on UA-DETRAC using Faster R-CNN (ResNet-50). 
% \vspace{-10pt}
% \begin{table}[!htb]
% 	\large
% 	\begin{center}
% 		\resizebox{\columnwidth}{!}{
% % 		\vspace{-10pt}
%     \begin{tabular}{||c | c | c | c| c ||} 
%     \hline
%     Hard samples & the best exiting strategy & mAP (\%) &  Flops (GFLOPS) & Throughput (img/s) \\  
%     \hline\hline
%     Top 0-20\% &  $B^{1}\cdot G^{5}$ & 78.44\% & 334.44 & 4.43 \\ 
%     \hline
%     Top 20-40\% & $B^{2}\cdot G^{4}$ & 75.32\% & 243.62 & 7.12 \\
%     \hline
%     Top 40-60\% & $B^{3}\cdot G^{3}$ & 79.12\% & 185.75 & 9.61 \\
%     \hline 
%     Top 60-80\% & $B^{4}\cdot G^{2}$ & 76.39\% & 145.29 & 11.23 \\
%     \hline
%     Top 80-100\% & $B^{5}\cdot G^{1}$ & 81.93\% & 125.37 & 12.59 \\
%     % 2 & 7 & 78 & 5415 \\
%     % \hline
%     % 3 & 545 & 778 & 7507 \\
%     % \hline
%     % 4 & 545 & 18744 & 7560 \\
%     % \hline
%     % 5 & 88 & 788 & 6344 \\ [1ex] 
%     \hline
%     \end{tabular}}
%     \end{center}
% % 	\vspace{-10pt}
% 	\caption{NN profile using Faster R-CNN (ResNet-50) on UA-DETRAC~\cite{CVIU_UA-DETRAC}. $B^{(5-i)}\cdot G^{i}$ denotes executing $i$ enhancement blocks and skip $(5-i)$ backbone blocks in downstream object detection.} 
% 	\vspace{-10pt}
% 	\label{table:profile_faster_rcnn}
% \end{table}
% \subsubsection{Instance distribution extraction} 
% \vspace{-15pt}
% To meet variants of hard samples, we need to record all difficult-levels of recent hard samples and update NN profile periodically. As illustrated in Figure~\ref{fig:overview}, we record difficult-levels of recent $w$ hard samples and send its cumulative distribution function (CDF) to performance estimation, in which it is easy to find recent difficult-level thresholds for Top xx-xx\%.
% % Heuristic relevant features of enhancement (scale, occlusion ratio, truncation ratio and accelerating ratio).  
% \subsubsection{Performance estimation}
% % \vspace{-15pt}
% With recent CDF, performance estimation module is responsible for updating NN profile with new difficult-level thresholds and finding the best exiting strategy for five groups of hard samples again.
% \subsubsection{Enhancement planning (scheduling)}
% Given a resource budget and recent NN profile, we need to change intervals of five groups adaptively and update the best exiting strategy again. An intuitive approach is to leverage the reciprocal of resource requirements of exiting strategies. For example, if resource requirements of $B^{1}\cdot G^{5}$ to $B^{5}\cdot G^{1}$ is 10, 6, 4, 3 and 1, we will set the proportion of five intervals to $\frac{1}{10}:\frac{1}{6}:\frac{1}{4}:\frac{1}{3}:1$.

==> tex/intro.tex <==
\section{Introduction}
\ys{1. Prevalence of cascaded pipeline in edge video analytics (e.g., motion detection + DNN object detection for counting tasks). 2. Dynamic compute workload due to video content variations vs. dynamic edge resource availability. 3. Adaptive image enhancement that maximizes analytics accuracy while at the same time smooths out resource utilization of any video analytics pipeline, making edge resource scheduling easier. 4. How multi-exit models fall short. }

\yan{(background) Object detection is very important to many video analytics applications (\textit{i.e.,} vehicle counting, pedestrian detection). Driven by recent breakthrough in Deep Neural Networks (DNNs) and the emergence of AI accelerators, state-of-the-art object detection techniques achieve awesome performance on many benchmarks. But DNN-based algorithms are often known to be computation-expensive and high computation cost, which lead to high processing latency and energy consumption.}

\yan{(compression and multi-capacity) To reduce this computation overheads, most researchers leverage deep compression techniques to generate more compact and efficient DNNs. Because the compression process is a one-time effort, these networks are also called \textit{one-size-fits-all} models. Unfortunately, using them to replace heavy DNNs completely often brings a significant performance drop on many difficult samples because most compact models are more sensitive to data drift or hard samples than large ones. To address this challenge, cascade models are widely used to adapt to the different difficult levels of input data. In video analytics, Chameleon~\cite{jiang2018chameleon} is proposed to change the DNN models dynamically based on recent profile results. In image classification, Cascade-inference~\cite{enomoto2021cascadeInference} is designed to learn an effective confidence calibration for selecting which samples are hard ones and are required to be further processing. Because cascade models contain many model variants, this kind of approaches is also called \textit{multi-model-variant methods}. Although they achieve better performance than \textit{one-size-fits-all} solutions, searching and switching the optimal model at runtime are often prohibitively expensive~\cite{fang2021flexdnn}. Thus, designing a single network with flexible complexities is crucial to input-adaptive applications.}

\yan{(early-exiting) Recently, a new interesting mechanism named \textit{early-exiting} has attracted more attention. It leverages computational redundancy of DNNs to add multiple exiting branches to original models. With such branches, easy samples exit in shallow layers and hard samples are processed with later layers. The key idea behind their operation lays on the fact that such features on easier samples might be enough to offer the desired distinguish-ability between class. Unlike \textit{multi-model-variant methods}, it doesn't need to search and switch the optimal model during the runtime because most of exiting policy is based on rule-based (\textit{i.e.,} confidence-criteria) and each sample will be sequentially analyzed. Thus, \textit{early-exiting} mechanism can be seen as promising light-weight solution for input-adaptive analytics. However, they are limited to three key drawbacks in many applications: (1) previous works designed exiting policy based on heuristics only, and they needed to process many unnecessary branches before the correct exit; (2) the number and locations of inserted early-exits are also decided by heuristic methods; (3) almost all prior works~\cite{enomoto2021cascadeInference, han2021dynamic} were designed for image classification, and they are hard to apply instance-level vision tasks (\textit{i.e.,} object detection).}

\todo{how to insert descriptions about GAN (image enhancement) before our solution?}

\yan{(our solution) In this paper, we present a novel instance-level DNN-based visual analytics framework named \name that leverages multi-exit image enhancement to adjust computation resources on different difficult-level images. \name runs a \textit{tailored} and \textit{multi-capacity} GAN-based enhancement model \textit{selectively} on incoming images to maximize the overall video analytics accuracy under the constraints of inference latency. Figure \ref{fig:example_adaptiveDet} shows an example of our key idea behind \name for vehicle detection on the MIO-TCD dataset~\cite{luo2018miotcd}.}

% \yan{(Comparison with domain adaptation techniques) 1. Prevalence of object detection in edge video analytics (\eg RoIs detected by object detection can be used in many downstream tasks, such as counting and reID). 2. Applying object detection models to a new domain is very challenging due to large domain shifts. To reduce this, ML researchers often use domain adaptation or labeling+training (supervised) methods. 3. However, some difficult domains (blur, lighting conditions) caused by moving cameras are not easy to adapt by existing training-based techniques because of small inter-class similarities (hard to annotate) and irregular occurrences (hard to switch models).}

% \yan{(Existing solutions) 1. Leverage domain knowledge to design an specific model using many training tricks and constraints (such as geometry and optical flow in video); 2. Add image enhancement modules (GAN) before object detection. The first method is rarely used in practice because it assumed that ML engineers have enough expert knowledge to choose correct constraints. The second approach ignores limits/requirements (resource-constrained, dynamic resource allocation) from \textbf{real-world deployments}. Most edge devices are hard to support a large computation burden of GAN+detection. Intuitively, we can also leverage existing early/multi-exit techniques to optimize GAN. But it is not easy to add exits because of a large search space of exits in diverse model architectures.}


% \yan{(Problem formulation) To design efficient and flexible image enhancement module for existing object detection models, we propose \name, a flexible multi-exit framework that can adaptively adjust computation resources across "easy" and "hard" inputs of image enhancement based object detection. \name runs a \textit{tailored} and \textit{multi-capacity} GAN-based enhancement model \textit{selectively} on incoming frames to maximize the overall video analytics accuracy under the constraints of inference latency. Figure \ref{fig:example_adaptiveDet} shows an example of our key idea behind \name for vehicle detection on the MIO-TCD dataset~\cite{luo2018miotcd}.}
\begin{figure}[!t]
	\begin{center}
	   \includegraphics[width=1.0\columnwidth]{Images/adaptiveDet_illustration.pdf}
	\end{center}
    \vspace{-10pt}
    \caption{An illustration of \name for vehicle detection on 3 frames from MIO-TCD~\cite{luo2018miotcd}. Purple, green and red arrows indicate different inference workflows for 3 frames respectively.}
    \vspace{-10pt}
	\label{fig:example_adaptiveDet}
\end{figure}

(Challenges and solution) Design of \name, however, faces three key technique challenges. First, a multi-exit GAN is not easy to train because it often suffers from two major problems: destabilize gradients of the mini-max game and diminished gradients caused by very strong discriminators. Thus, it is non-trivial to train a stable multi-exit GAN for the downstream object detection task. Second, training a multi-exit GAN often brings a large computational burdens due to the huge search space of resolution and channel selection~\cite{lin2021anycost}. Also, the architecture of current multi-exit GANs is not efficient for real-world deployment because we have to run many unnecessary layers (exits) before we find the correct exit. Third, executing multi-exit GAN effectively requires the awareness of dynamic resource capacities and the NNs' capacities, which are unknown and hard to predict. To address the first issue, \name leverages detection loss to constrain the unstable mini-max optimization and builds two-level (image-level and instance-level) discriminators to avoid diminished gradients caused by a single and strong discriminator. To reduce large training burdens and design inference-friendly multi-exit architectures, \name reuses backbone layers from object detection models as an encoder in the generator of GAN and only fine-tunes the decoder layers. Benefiting from multi-scale discriminative features extracted by backbone layers, generators are easy to create multi-scale enhanced images. Besides, we leverage the instance-level discriminator from GAN to get more accurate difficult-level for a new image and use it to decide the optimal exit, best balancing the trade-off between accuracy and resource budget. To meet the dynamic resource budgets, \name builds three kinds of resource-driven schedulers (flops/latency) to adjust the enhancement strategy for an given image. It first builds an offline profile to record flops/latency of different exiting strategy. In online executing, it takes the cumulative distribution function (CDF) of difficult-level history and a new predicted difficult-level as input, and leverage a suitable resource-driven scheduler to find the exiting strategy for a new image to maximize detection accuracy under the given resource budget. In summary, the main contributions are as follows: 
% \vspace{-2pt}
\begin{itemize}
    \item We first propose \name, a flexible and efficient image enhancement for object detection. \name makes the best of edge computing resources and runs off-the-shelf object detection networks with enhancement modules (GAN) at a fine-grained level of latency and accuracy.
    \item We design and implement the detection-driven training strategy, a effective and fast learning strategy to train enhancement modules without modifying object detection models. This strategy leverages backbone layers' characteristics to find the optimal exit for enhancement modules, and use detection loss to learn effective sharing features between backbone and enhancement modules.
    \item We evaluate \name on two real-world traffic images. Evaluation results show that \name achieve xxx\% speedup with an accuracy drop of xxx\% from the state-of-the-art (SOTA) enhancement-based object detection pipelines. In addition, \name obtains xxx\% detection accuracy improvements on average, compared with SOTA techniques under the same latency constraint.
\end{itemize}
% C1: How to decide exits of GAN architectures? (detection-driven design in co-training); C2: How to take downstream detection task into account during enhancement? Because existing GAN modules are only responsible for generating high-quality images (detection-GAN co-training, feature reuse); C3: How to decide multi-exits for incoming new images? (resource-driven threshold scheduler, flops-based/latency-based/energy-based)}




% We are witnessing unprecedented investment and development in the space of live video analytics with the advancement of artificial intelligence and the proliferation of cameras. Recently, an increasing number of real-time video analytics scenarios require analyzing video in smart cameras or other edge devices due to the limited latency requirements. In video analytics applications, object detection plays a pivotal role because of its ability to identify and localize all objects/instances of certain categories in an image. It also serves as a basic task for many high-level vision tasks (\textit{i.e.,} object counting, re-identification, tracking, anomaly detection and natural language-based object retrieval).  

% Although a number of deep convolutional neural network (CNN) based object detection techniques have achieved excellent performance on many benchmark datasets, they are limited by out-of-distribution (OOD) data which is rarely or never present in the training data. For example, small-size or high-speed vehicles are hard to detect by existing object detection models because it's difficult to collect precise annotations for these objects in the training data. In machine learning, a naive and widely used approach to address the OOD issue is leveraging semi-supervised training~\cite{jin2018semiod} to train detection models on labeled normal data and unlabeled anomaly data. However, this kind of approaches is offline and difficult to achieve enough better performance in many challenging environments with numerous unlabeled anomaly data. As the development of generative adversarial network (GAN) based image enhancement (IE), an recently effective method to resolve the OOD problem under challenging and complex environments (\textit{i.e.,} low-light, hazy and underwater images) is IE-based object detection~\cite{islam2020FUGan,xin2021detection}, in which IE enhances each image before object detection. Unfortunately, it brings inevitable large computational costs~\cite{li2020gancost,lin2021anycost} for running a IE models on each frame in resource-constrained edge devices. 

% To fill this gap between the needs of fast and accurate IE-based object detection on incoming videos and the limited resources on edge devices, we propose \name, a flexible multi-exit framework that can adaptively adjust computation resources across "easy" and "hard" inputs of IE-based object detection. \name runs a \textit{tailored} and \textit{multi-capacity} GAN-based enhancement model \textit{selectively} on incoming frames to maximize the overall video analytics accuracy under the constraints of inference latency. Unlike existing multi-exit solutions that select frames based on heuristic image classifiers, \name builds instance-level classifiers trained from unpaired detection-driven GAN on incoming videos at a fine-grained level of latency and accuracy. Figure \ref{fig:example_adaptiveDet} shows an example of our key idea behind \name for vehicle detection on the MIO-TCD dataset~\cite{luo2018miotcd}.
% \begin{figure}[!t]
% 	\begin{center}
% 	   \includegraphics[width=1.0\columnwidth]{Images/adaptiveDet_illustration.pdf}
% 	\end{center}
%     \vspace{-10pt}
%     \caption{An illustration of \name for vehicle detection on 3 frames from MIO-TCD~\cite{luo2018miotcd}. Purple, green and red arrows indicate different inference workflows for 3 frames respectively.}
%     \vspace{-10pt}
% 	\label{fig:example_adaptiveDet}
% \end{figure}

% Our key insight is that not all instances are required to be enhanced fully. Some hard instances only need a little of discriminative details to be reconstructed to easy instances. 

% Based on it, design of \name faces three main technical challenges. First, it's difficult to distinguish "easy" and "hard" inputs without any annotations. Existing multi-exit deep neural networks build classifiers on many heuristic methods which might face the issues of overconfidence, high sensitivity for threshold setting and poor transferability. Second, current GAN based IE models are high resource-demanding that makes them unsuitable for many resource-constrained edge devices. Third, executing IE-based object detection at various latency budgets requires the awareness of variants of video content. For example, a sudden change of objects should attract more attention than other variants in anomaly detection. To cope with the first and second issues, we design a detection-driven IE model which uses backbone modules from off-the-shelf object detection models as encoders of the generator in raw GAN-based IE model. To get better transferable feature maps for downstream detection tasks, we use a extra detection loss to train the generator of our driven-based IE. Benefiting from unpaired adversarial training, we obtain effective discriminators or classifiers after GAN training which are able to distinguish anomaly instances. To deal with variants of video contents, \name leverages an effective performance estimator to predict enhancement's performance under different instance-level variants (object distributions) based on previous detection results and generates an optimal selection strategy across an efficient scheduler which takes the latency budget and the performance estimation as inputs to decide which exit can be triggered for each frame of a given video. In summary, our contributions are as follows:
% \begin{enumerate}multi-scale
%     \item We design a novel detection-driven multi-exit IE model with coarse-to-fine discriminators/classifiers. Based on it, \name is able to make the best of edge compute resource and improve off-the-shelf object detection networks on any given videos at a fine-grained level of latency and accuracy.
%     \item We build an efficient and effective scheduler to select exit layers dynamically for all frames of a given video. Based on the selection strategy, \name achieve better overall performance than other image enhancement based object detection under the latency budget at runtime. 
%     \item We implement \name on a \textbf{Jetson} edge device and evaluate it on multiple traffic video datasets. Evaluation results show that ...
% \end{enumerate}

==> tex/motivation.tex <==
\section{Motivation and Background}

\ys{Instead of talking about multi-exit and GAN, we should start the motivation by showing the potential of the judicious use of image enhancement. More specifically, applying IE on a small portion of images (e.g., hard samples) could lead to a drastic increase of detection accuracy. Next, we introduce existing IE approaches especially GAN-based ones and their limitations.}

\yan{(Measurement) 1. Hard samples in datasets (category, unpredictable, transient and spread in the time); 2. Existing solutions to address hard samples (supervised-training under specific settings or image enhancement); 3. Opportunities;}

\sq{Goal: Discuss hard samples \& instances in real cases, and show the image enhancement (IE) can help. Applying IE on these hard samples can lead to a drastic increase of detection accuracy, with little cost. (0) what are the hard sample \& instance? For a model, if it cannot detect the instance successfully (confident score < 0.5), or detected IoU < 0.5, it is a hard instance for this model. (1) on COCO dataset, use COCO-pretrained model, demonstrate hard instances and analyze their causes; (2) on traffic dataset, use COCO pre-trained model, demonstrate hard instances; (3) on traffic dataset, use fine-tuned \& re-trained model, demonstrate hard instances; (4) apply IE; (5) retrain v.s. IE, complementary, in terms of accuracy gain and computation power cost.}

\subsection{Instance-level content dynamics \& Benefit of using IE}
Due to mobility of cameras, videos taken in real-world mobile settings exhibit substantial content dynamics in terms of difficulty level across frame over time. Such dynamics often make DNN-based models performance drop because their static computation pipelines are hard to adapt on changing variants from real-world applications. To meet dynamics, some researchers propose multi-exit networks to adjust computation pipeline for different input data. However, they only focus on image-level applications and are hard to extend on instance-level jobs. For example, it is non-trivial to decide easy/hard characteristics for a image with a few hard samples (as shown in Figure~\ref{fig:instance_level}, only one high-speed car is assigned to a wrong class). 
\begin{figure}[!t]
	\begin{center}
	   \includegraphics[width=1.0\columnwidth]{Images/instance_level.pdf}
	\end{center}
    \vspace{-10pt}
    \caption{An illustration of hard samples in object detection.}
    \vspace{-10pt}
	\label{fig:instance_level}
\end{figure}
To explore potential of enhancement model on this instance-level dynamics, we run IE and detection models on different subsets of hard samples from MIO-TCD-2018 dataset~\cite{luo2018miotcd}. Figure~\ref{fig:potential_IE} shows the end2end performance (mAP) for YOLOv3~\cite{yolov3} using enhancement on top-10\%, top-20\%, top-30\%, top-40\% and random-10\% hard samples~\footnote{In this experiment, we use ground-truth to annotate hard samples for testing data.}. It's interesting to note that top-30\% perform best of all methods and only random-10\% is worse than YOLOv3~\cite{yolov3}. To find why top-40\% is lower than top-30\%, we add a supervised training method as the upper-bound to Figure~\ref{fig:potential_IE}.
\begin{figure}[!t]
	\begin{center}
	   \includegraphics[width=1.0\columnwidth]{Images/potential_IE.eps}
	\end{center}
    \vspace{-10pt}
    \caption{mAP of using different IE strategies on MIO-TCD-2018~\cite{luo2018miotcd}.}
    \vspace{-10pt}
	\label{fig:potential_IE}
\end{figure}
\subsection{Over-provisioned GPU resources}
\yan{(Metrics for GPU utilization) There are two key metrics on GPU utilization: GPU busy time (temporal) and streaming multiprocessor efficiency (spatial). Because GPU busy time denotes the time during execution process where there is at \textbf{one kernel} running on it, it is often seen as a coarse-grained metric and hard to ... In contrast, streaming multiprocessor (SM) efficiency can profile GPU utilization accurately because it sums all SM utilization of each step time. In a step time, higher SM utilization means more GPU kernels are activated for the current job. Thus, high SM efficiency denotes better GPU utilization. \\(Reasons for over-provisioned GPU resources) Although light-weight models are widely used in edge devices, there is still existing many redundant GPU resources during inference due to executing a small model with fixed batch-size.\\ (Existing solutions to improve GPU resources) xxx\\(Advantages for leveraging Image Enhancement) It Motivates us to find specific objectives...} 
\subsection{Existing IE techniques}
While IE is promising to address dynamics caused by moving cameras, existing methods are too computation-expensive and \textit{misfit} to resource-constrained edge systems. This is because only a few GAN-based acceleration techniques~\cite{hou2021slimmGAN, lin2021anycost} are proposed and their implementation is often costly. More important, all of them define easy/difficult characteristics based on resolution. AnyCost-GAN~\cite{lin2021anycost} is the first proposed dynamic GAN, which leverages neural architecture search (NAS) to filter unimportant convolutional channels to speed up inference. Although NAS is a effective tool to search compact models, its heavy learning cost is unbearable for many resource-constrained systems.
% \begin{figure}[!t]
% 	\begin{center}
% 	   \includegraphics[width=1.0\columnwidth]{Images/multi_exit_gan.pdf}
% 	\end{center}
%     \vspace{-10pt}
%     \caption{An illustration of the generator in anyCost-GAN. Red, green and purple arrows denote 3 inference workflows for 3 different images.}
%     \vspace{-10pt}
% 	\label{fig:anycost}
% \end{figure}
% We begin with introducing existing multi-exit techniques and summary their limitations.

% % In previous works, heuristics which are widely used are confidence-criteria and rule-based approaches (\textit{i.e.,} determined by the entirely objects is whether in a given image or not). For instance-level tasks, each region-of-interest (RoI) may have a distinct confidence-prediction and scores assigned by rules (\textit{i.e.,} size and occlusion ratio). Thus, how to analyze a group of results is crucial to implement effective early-exiting. Figure xxx shows two images sampled from traffic videos in xxx using occlusion ratio as the rule. We find that the left image has high performance (mAP) but is assigned to a lower difficult-level.

% % The benefits from image enhancement are caused by adding more distinguishable semantic details to hard samples. To measure this gain, we compare mAP of Faster-RCNN~\cite{} and enhancement+Faster-RCNN~\footnote{we use this enhancement to generate high resolution images for Faster R-CNN.}. In this experiment, we use HRNets~\cite{} as our enhancement module, and also plot the upper-bound of Faster-RCNN that is achieved by fine-tuning with ground-truth.
% \subsection{Main challenges of multi-exit GAN}
% Although mult-exit mechanisms are successfully applied to convolutional neural networks (CNN) and recurrent neural networks (RNN), there is existing very little works~\cite{hou2021slimmGAN, lin2021anycost} on multi-exit GAN. Compared with CNN and RNN, GAN is hard to train because of destabilize and diminished gradients from mini-max games. The new SOTA named anyCost-GAN~\cite{lin2021anycost} is the first multi-exit GAN, which integrated with distillation~\cite{yu2020distill, wang2020distill}, neural architecture search (NAS)~\cite{li2020nas, fu2020nas}, adaptive-channel~\cite{hou2021slimmGAN} and multi-scale feature fusion~\cite{karnewar2020multiscalegan} techniques. As shown in Figure~\ref{fig:anycost}, anyCost-GAN~\cite{lin2021anycost} achieves an dynamic or flexible inference through adaptive channel selection and multi-resolution outputs. Unfortunately, finding the suitable channel in each layer and the optimal resolution for new inputs is still a difficult problem because of a huge search space. While they leverage NAS to complete search tasks, it is hard to update search strategy dynamically under new resource budgets because of a large computational cost of NAS. Besides, they don't provide a clear practical guide on how to use it in current object detection inference workloads. Intuitively, we add an image classifier before anyCost-GAN to decide which layers/channels should be skipped in GAN. But in practice, it is difficult to obtain the best exiting strategy based on image-level features because there is existing many instance-level variants between two similar images on image-level. For instance, two dark images may contain different number of region-of-interests (RoI). In summary, there are two main challenges behind multi-exit GAN design: (1) dynamic architectures are hard to search and update; (2) dynamic GAN requires a more fine-grained level classifier to decide the optimal exiting strategy.
% \begin{figure}[!t]
% 	\begin{center}
% 	   \includegraphics[width=1.0\columnwidth]{Images/multi_exit_gan.pdf}
% 	\end{center}
%     \vspace{-10pt}
%     \caption{An illustration of the generator in anyCost-GAN. Red, green and purple arrows denote 3 inference workflows for 3 different images.}
%     \vspace{-10pt}
% 	\label{fig:anycost}
% \end{figure}
% \vspace{-10pt}
% \subsection{Opportunities}
% The above challenges drive us to design more an efficient and effective multi-exit GAN to improve accuracy of downstream high-level vision tasks (\eg object detection and segmentation) under dynamic resource budgets. We argue that existing multi-exit GAN is a promising approach to accelerate enhancement processes but it ignores correlations between enhancement and post-processing tasks.
% In object detection models, backbone layers are often responsible for extracting discriminative features for an image and they serve as an encoder in anyCost-GAN~\cite{lin2021anycost} (the left part of Figure~\ref{fig:anycost}). Benefiting from many multi-scale training strategies~\cite{yu2018multiscale, guo2020multiscale}, backbone layers can also extract multi-scale features which decoders  required in Figure~\ref{fig:anycost}. Thus, an straightforward approach to design multi-exit enhancement modules for object detection is reusing backbone layers of detection models as an encoder and creating new CNN layers to process multi-scale features as the decoder. The advantages of this detection-driven design are threefold. First, it is easy to integrate with many instance-level classifiers after backbone layers to decide the optimal exit for decoders. Second, we can train or update multi-exit GAN fast and efficiently due to multi-scale discriminative features extracted by backbone layers. Third, this detection-driven enhancement modules can be seen as a play-and-plug component and is easy to integrate with any object detection models.
% that splitting enhancement and post-processing tasks is an effective to many practical applications 
% This section explores three questions: (1) Why we choose GAN as ? (2) how does GAN improve performance on hard samples? (3) what compute/memory resources does naive GAN require?
% \yan{1. Why we choose GANs as image enhancement models (because GAN is very general than other specific enhancement methods)? 2. Why existing GANs are not used in edge video analytics (measurement on popular GAN-based image enhancement models)? 3. Why we choose detection-driven to decide exits in GAN instead of using other multi-exit techniques?}
% \subsection{Impacts of existing GAN on hard samples}
% xxx
% \subsection{Limitation of GAN}
% xxx

==> tex/motivation2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/dynamic_workloads-crop.pdf}
    \caption{An illustration of an edge video analytics pipeline, and its workload dynamics caused by the temporal pruning optimization.}
    \label{fig:illustration_vap}
\end{figure}

\section{Motivational Study}
\label{sec:motivation}
% \ys{Instead of talking about multi-exit and GAN, we should start the motivation by showing the potential of the judicious use of image enhancement. More specifically, applying IE on a small portion of images (e.g., hard samples) could lead to a drastic increase of detection accuracy. Next, we introduce existing IE approaches especially GAN-based ones and their limitations.}

% \yan{(Measurement) 1. Hard samples in datasets (category, unpredictable, transient and spread in the time); 2. Existing solutions to address hard samples (supervised-training under specific settings or image enhancement); 3. Opportunities;}

% \sq{In this section, we talk about the motivation and demonstrate some preliminary study results. Logical chain 1) There exist idle resources in current video analytics pipelines on edge (why exist); 2) Such idle resources appear erratically, unpredictably; 3) To best utilize the idle resources, we need a plug-and-play approach, and the image enhancement shows the potential; 4) Illustrate the object detection performance when applying IE, discuss our key observation, that is proper IE method must be applied onto proper frame to guarantee the gains, otherwise no gains or even negative impacts are brought; 5) However, such the selection is very difficult, demonstrate the experiment results, reveal the best selection is the frame-level and detector specific. 6) Based on the insights, propose the design principles.}



\subsection{Over-provisioned Compute Power}
% \sq{In this sub section, we talk about 1) idle resources exist in edge video analytics pipelines, and why they exist (over-provision); 2) the pattern of idle resources (erratically and unpredictably); 3) to utilize such idle resources, model-oriented approach is not efficient. It calls for a plug-and-play approach. The input-oriented approach, \ie image enhancement shows the potential.}
% \sq{Have to highlight hard samples, easy samples and something}

% 互补这个是我们之前想的主要论点。当然可以finetune原模型，但是这样并不解决我们所针对的idle resources闲置的问题。再好的模型也可以有通过我们的方法提升的空间(可以加个实验佐证)。

% \sq{For the causes of dynamic workload, DiStream (sensys'20) claims that it is due to different video analytics pipeline.}

% there are some residual resources
Edge devices are usually known to be resource-constrained, but in real-world deployments we notice edge compute power is often over-provisioned for video analytics. It is mainly due to the tension between the fixed hardware when deployed and the dynamic workload in run time.
% which is mainly due to pipeline optimizations.

% The residual resources are mainly due to the optimized video analytic pipelines. 

Fig.~\ref{fig:illustration_vap} demonstrates a typical video analytics system. Multiple cameras stream to an edge server, where downstream tasks, \ie object detection, are performed. When deploying the edge server, its compute power is carefully provisioned, enabling the system to process all possible workload from every camera. 

Recent years, numerous video analytics pipelines are proposed to optimize accuracy and cost trade-off~\cite{zhang2017live,noscope2017,awstream2018,glimpse2015,vigil2015,jiang2018chameleon,hung2018videoedge,Reducto,eaar2019}. For example, as shown in Fig.~\ref{fig:illustration_vap}, \emph{temporal pruning} is applied. It selectively drops frames based on heuristics (\eg significant differences between frames), which leads to workload dynamics. In addition to temporal pruning, optimizations including \emph{spatial pruning} (\eg region cropping and background extracting) and \emph{model pruning} (\eg model selection and specialization), have been widely integrated with the video analytics pipelines~\cite{measurement2021xiao}. The edge compute power is usually fixed once deployed 
but the workload is dynamic. Thus there would be probably over-provisioned compute power at times for current edge video analytics system.

% Thus the pipeline optimizations lead to workload dynamics.
% While in practice, pipeline optimizations are usually applied. For instance, because of the temporal pruning~\cite{}, some of frames would be not be processed probably, leading to lighter workload. Therefore the compute power is over-provisioned and residual resources come out at times.
% The compute resources of the edge cluster are usually configured to be capable to process the full workload from all connected cameras. However, due to the pipeline optimizations, \eg temporal pruning~\cite{}, some frames might be skipped. Therefore the compute power is over-provisioned at times. \todo{add symbols according to the figure}
% Besides the temporal pruning, there are also many other optimization techniques, \eg spatial pruning~\cite{} and model pruning~\cite{}. They have been widely integrated with current edge video analytic pipelines nowadays, and led to probable residual resources~\cite{}.

% \sq{switch to a larger model}

We identity the opportunity that residual resources could be utilized to in further improve inference accuracy. However it exposes new challenges to capture such over-provisioned compute power on edge video analytics systems.
% Intuitively, over-provisioned compute power can be used to fine-tune or retrain deployed models~\cite{}. However end-to-end model optimizations might not be appropriated, because residual resources are insufficient for the backward propagation progress.
% To facilitate it, we study the workload dynamics as well as the video analytics accuracy
% Thus we firstly analyze the characteristics of the residual resources.

\begin{figure}[t]
    \subfigure[Vigil]
    {
        \includegraphics[width=0.46\linewidth]{Figures/dynamic_resources_vigil-crop.pdf}
        \label{subfig:dynamic_vigil}
    }
    \hfill
    \subfigure[Glimpse]
    {
        \includegraphics[width=0.46\linewidth]{Figures/dynamic_resources_glimpse-crop.pdf}
        \label{subfig:dynamic_glimpse}
    }
    \caption{Dynamic workload and corresponding idle resources of the edge video analytics system when integrating different temporal pruning methods.}
    \label{fig:dynamic_workload}
\end{figure}

\begin{figure*}[!t]
\begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/enhancement_gain-crop.pdf}
        \caption{Overall mAP of EfficientDet on raw and enhanced images from  UA-DTRAC.}
        \label{fig:overall_accuracy_with_without_ie}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/enhancement_per_image-crop.pdf}
    \caption{mAP on every raw \textit{(blue)} and enhanced \textit{(orange)} image of a selected video trace. }
    \label{fig:accuracy_per_image_with_ie}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/enhancement_optimal_selection-crop.pdf}
    \caption{mAP on raw images and enhanced images with the optimal selection.}
    \label{fig:accurac_optimal_selection}
\end{minipage}
\end{figure*}

Fig.~\ref{fig:dynamic_workload} showcases the dynamic workload traces and corresponding idle resources when when processing 6 video streams at 25 FPS on a edge server for 80 seconds. We integrate two popular temporal pruning methods with this video analytics pipeline, Vigil~\cite{vigil2015} and Glimpse~\cite{glimpse2015}, as shown in Fig.~\ref{subfig:dynamic_vigil} and~\ref{subfig:dynamic_glimpse}, respectively. Overall due to the temporal pruning, XX\% and XX\% workload are dropped on average, for Vigil and Glimpse, which leads to idle resources. Furthermore we notice the workload varies dramatically. For example, it is up to XX\% and for Vigil. 
% Video streams are required to be processed in time, the residual resources in the current processing window are hardly carried into next windows, due to the agnostic workload.
In addition, the workload dynamics are mainly due to video content fluctuations, thus the distribution of the over-provisioned compute power is fragmented and usually unpredictable.

% Such dynamics are mainly due to video content fluctuations. What's more, we observe the over-provisioned compute power caused by the workload dynamics is often fleeting, fragmented and unpredictable. \sq{too weak, more reasoning?}


% the workload dynamics and corresponding over-provisioned resources of an object detection pipeline, performing EfficientDet~\cite{} on six video streams, and integrated with the temporal pruning on a Nvidia Jetson.~\todo{update the real example}. We notice that the workload varies dramatically, from to XX\% to XX\%. What's more, such dynamics are mainly due to video content fluctuations, making the residual resources variable, unpredictable and fragmented.

End-to-end model optimizations, \eg fine-tuning and retraining, fall short of capturing the over-provisioned resources. Improving models usually requires a vast compute power, while the residual resources are fragmented and unpredictable. It is too difficult to breakdown the model training process and distribute properly to fit the idle resources. 


To best utilize the opportunistic idle resources, it calls for a flexible, fine-grained, plug-and-play approach. Instead of improving models, we shift our focus on enhancing inputs, \ie applying image enhancement approaches.


% What's more, the appearances of residual resources are unperiodically, fragmented, since the dynamic workload is caused by the video content fluctuations, which are too difficult to predict.\todo{give numbers.}
% To utilize the opportunistic resources, directly applying end-to-end model optimization methods, \eg picking larger models~\cite{}, and fine-tuning deployed models continuously~\cite{}, etc, might not be appropriate.\todo{give reasons.}
% Therefore, best utilizing the opportunistic resources calls for a flexible, fine-grained, plug-and-play solution. To this end, we shift our focus from the model optimizations to the input optimizations, \ie image enhancement~\cite{}.
% Intuitively, we could make use of these resources to optimize DL models, \eg applying larger models~\cite{}, and fine-tuning deployed models continuously, etc. The model-oriented optimization approaches, however, might not be appropriate. Caused by the video content fluctuations, opportunistic residual resources are usually un
% However it is difficult to directly apply existing model optimization methods, including scaling-up models, retr
% should be utilized to in further improve the detection results. To this end, a wide range of approaches are discussed~\cite{}, including up-scaling models~\cite{}, continuously retraining and fine-tuning models~\cite{}, etc.
% Such model-oriented optimization approaches, however, are not always appropriate for edge video analytic pipelines \sq{in this scenario}. Dynamic workload caused by the video content fluctuations makes edge resource usage non-deterministic and unpredictable, while end-to-end model optimization methods are not flexible enough meet such resource dynamics. For instance, Fig.~\ref{} demonstrates the GPU utilization when \todo{Give an idle resources example}.
% Therefore, to best utilize the opportunistic idle resources, it calls for a flexible, fine-grained, plug-and-play approach. Instead of optimizing models, the input-oriented optimization approaches, \ie image enhancement, show their potential.\todo{maybe some reasoning?}

% \sq{In this sub section, we talk about 1) experiment setup, dataset and IE approaches; 2) Overall results, IE shows the very limited gains; 3) Analysis in depth, demonstrates mAP gains over scenes and in typical scenes; 4) Our key observation, IE bring gains only if we apply best selection.}
\subsection{Image Enhancement}
% Zamir2021MPRNet (deblurring, deraining), liang2021swinir (denosing, ), qin2020ffa (dehazing), jiang2021enlightengan (light), Zero-DCE2020 (light)
% what is image enhancement
Image captured in real world might suffer from poor visibility, low contrast and high noise, etc. These issues challenge both human visual perception as well as video analytics systems. To mitigate the degradation, a number of image enhancement algorithms are proposed, ranging from histogram based ones~\cite{2005histogram} to deep learning based approaches~\cite{Zamir2021MPRNet,liang2021swinir,qin2020ffa,jiang2021enlightengan,Zero-DCE2020}.
% image enhancement for video analytics
Image enhancement methods, \eg super resolution, deblur and dehaze, etc, are enable to restore corrupted details in raw captured images, in turn they could benefit downstream tasks in video analytics systems, \ie classification~\cite{distream2020sensys} and object detection~\cite{noscope2017}.
% why image enhancement --> Immediate impacts, best utilize the idle resources
In addition, image enhancement methods potentially fits the characteristics of over-provisioned compute power. Unlike training methods, the image enhancement applies optimizations on each input. Such the image-level enhancement is fine-grained. We could easily determine the amount of inputs that would be enhanced, according to the idle resources. In this way, the over-provisioned computer power can be fully utilized and the downstream task can obtain immediate improvements.

% In order to fully utilized the idle resources, we can determine how many inputs could be enhanced accordingly.

% By applying image-level enhancement, the optimizations have immediate improvements on downstream tasks.  The input-oriented method is elastic to utilize the fleeting, fragmented and unpredictable ideal resources.
% study on image enhancement for video analytics

To explore the potential of integrating video analytics with image enhancement, we conduct a preliminary study. We select six types of image enhancement methods, including super resolution (SR)~\cite{liang2021swinir}, dehaze~\cite{qin2020ffa}, deblur~\cite{Zamir2021MPRNet}, denose~\cite{liang2021swinir}, relight~\cite{jiang2021enlightengan, Zero-DCE2020} and derain~\cite{Zamir2021MPRNet}. We make use of UA-DETRAC~\cite{CVIU_UA-DETRAC} as our measurement dataset. It contains more than 100 video clips with rich annotations, \ie vehicles and pedestrians. The videos are captured from real-world traffic scenes at multiple locations under different environment conditions. We take the object detection as an example downstream task. We use EfficientDet-D0~\cite{efficientdet2020} as the object detector. We take the mean average precision (mAP) as the measurement metric, and we have the following observations.

% key observations
% 1) simply apply image enhancement cannot get gain
% 2)

Firstly, we observe that solely applying image enhancement methods brings very limited accuracy gains for video analytics. Fig.~\ref{fig:overall_accuracy_with_without_ie} illustrates the overall mAP on raw and enhanced images of UA-DTRAC. We find the detector can hardly obtain better results on enhanced images. For instance, the deblur brings the biggest improvements, which is only about 0.7\%. For the relight method even has negative impacts on the detection, that lowers the mAP by 3\%.


Secondly, we observe that only a small portion of images need enhancements. Fig.~\ref{fig:accuracy_per_image_with_ie} demonstrates the phenomenon. It shows
the mAP of individual raw and enhanced image from a selected video trace, which contains about 480 frames. As shown, the enhancements can only bring gains for a portion of frames. Specifically, when applying the deblur and relight, the detection can improve only XX\% and XX\% of enhanced frames, respectively. 


Meanwhile, improperly applying enhancements not only bring no gains, even have negative impacts. For example, applying the dehaze on some frames, up to XX\% mAP would be decreased, compared to the detection on raw frames.\todo{talk about hard easy}

Thirdly, we observe that the judicious use of image enhancements could lead to a drastic increase of detection accuracy. We use the video trace in Fig.~\ref{fig:accuracy_per_image_with_ie}. For each image in this trace, we check if the enhancement is needed. If so, we always select the enhancement method that bring the most significant improvements. Fig.~\ref{fig:accurac_optimal_selection} shows the performance of such the optimal selection. Compared to the detection on raw images, the enhancements with optimal selection bring about more than XX\% mAP improvement on average, up to XX\%.

To summarize our preliminary study, we find that the image enhancement methods can improve the detection accuracy significantly, if and only if we select the proper portion of frames and apply the proper enhancement method. Otherwise the gain is very limited, even it may lead to the performance degradation.

% More, when applying the deblur and , only XX\% of enhanced frames can improve the detection. While


% frames can improve the detection. While for the super resolution

\subsection{Challenges and Opportunities}


Image enhancements show potentials of well utilizing the opportunistic residual resources on edge video analytics pipelines, and improving the downstream tasks. However, to eventually integrate image enhancements with video analytics, there are still several key challenges. And meanwhile we also reveal some opportunities.

Firstly, deep learning based image enhancement methods~\cite{} are usually too heavy to deploy on edge. For instance, the super resolution and the denoise take XX ms and XX ms per inference on a typical edge sever, Nvidia Jetson. They are even slower than the analytics tasks, \ie EffcientDet (XX ms). But we also notice that existing enhancement methods often focus on recovering the absolute image quality, which might be over-killed for the downstream tasks. The downstream tasks are often able to tolerate some levels of poor inputs. Therefore, considering the capability of the deployed task model, we have the opportunity to design a light but efficient enhancement method, especially for the particular model.
% \sq{In this sub section, we talk about 1) best selection is very difficult, show exp results; 2) best selection is scene-specific, and detector-specific; 3) to solve this problem, a co-design approach is needed.}

Secondly, according to our preliminary study, image enhancements work only if we apply the optimal selection, hence selecting the proper portion of hard frames and applying the proper enhancement. It is difficult to obtain such the optimal selection, because it is scene-specific and task-specific. Fig.~\ref{fig:optimal_selection_different} demonstrates an example where the optimal selections of 8 video traces are shown. For EfficientDet, the selections among traces are diverse. They highly accords with the particular video contents. Besides that, for the same video, the selections among different models are also very diverse, as shown in Fig.~\ref{fig:optimal_selection_different}.


Considering the challenges and opportunities above, we propose design a detector-specific image enhancement component, and integrate it with the object detection pipeline on edge.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/enhancement_showcase_selection-crop.pdf}
    \caption{The optimal enhancement selection of EfficientDet and YOLO on 8 selected video traces from UA-DTRAC.}
    \label{fig:optimal_selection_different_model}
\end{figure}

